Collaboration with Cellular Networks for RFI Cancellation at Radio Telescope

The growing need for electromagnetic spectrum to support the next generation (xG) communication networks increasingly generate unwanted radio frequency interference (RFI) in protected bands for radio astronomy. RFI is commonly mitigated at the Radio Telescope without any active collaboration with the interfering sources. In this work, we provide a method of signal characterization and its use in subsequent cancellation, that uses Eigenspaces derived from the telescope and the transmitter signals. This is different from conventional time-frequency domain analysis, which is limited to fixed characterizations (e.g., complex exponential in Fourier methods) that cannot adapt to the changing statistics (e.g., autocorrelation) of the RFI, typically observed in communication systems. We have presented effectiveness of this collaborative method using real-world astronomical signals and practical simulated LTE signals (downlink and uplink) as source of RFI along with propagation conditions based on preset benchmarks and standards. Through our analysis and simulation using these signals, we are able to remove 89.04% of the RFI from cellular networks, which reduces excision at the Telescope and capable of significantly improving throughput as corrupted time frequency bins data becomes usable.

==> ack.tex <==
\section*{Acknowledgement}
%\vspace{-5pt}
This work is funded by the National Science Foundation SWIFT Program (Award Number - 2128581).
%\vspace{-5pt}


==> additional.tex <==
\section{Additional Results}






\begin{comment}

\begin{figure*}[h]
\centering
\includegraphics[width=1\linewidth]{figs/uplink_block_rfi_updated.png}
\caption{Sample Uplink Scenrario}
    \label{fig:uplink_block}
    \vspace{-0pt}
\end{figure*}

\begin{figure*}[h]
\centering
\includegraphics[width=0.56\linewidth]{figs/illustration_UL_DL_channel.png}
\caption{RFI propagation from LTE cell: Uplink and Downlink}
    \label{fig:uplink_block_close}
    \vspace{-0pt}
\end{figure*}

\end{comment}



\begin{comment}
\begin{figure*}[h]
\centering
\begin{subfigure}[b]{0.4\linewidth}
    \includegraphics[width=\linewidth]{figs/macroCell_rqf.png}
    \caption{Urban Macro-cell}
    %\caption{\note{PSD of astro signal}\\\greg{use xlim() on all plots}}
    \label{fig:astro}
\end{subfigure}
\begin{subfigure}[b]{0.4\linewidth}
    \includegraphics[width=\linewidth]{figs/microCell_rqf.png}
    \caption{Urban Micro-cell}
    \label{fig:lte_psd}
\end{subfigure}
\begin{subfigure}[b]{0.4\linewidth}
    \includegraphics[width=\linewidth]{figs/ruralMacro_rqf.png}
    \caption{Rural Macro-cell} %\greg{get rid of this one?}}
    \label{fig:signals_time_domain}
\end{subfigure}
\begin{subfigure}[b]{0.4\linewidth}
    \includegraphics[width=\linewidth]{figs/suburbMacro_rqf.png}
    \caption{Suburban Macro-cell}
    \label{fig:composite_psd}
\end{subfigure}
\begin{subfigure}[b]{0.4\linewidth}
    \includegraphics[width=\linewidth]{figs/in2outdoor_rqf.png}
    \caption{Indoor to Outdoor Urban Channel}
    \label{fig:composite_psd}
\end{subfigure}
\caption{Reconstruction Quality in presence of RFI from Uplink Signal - Different Channel scenarios}
%I am guessing this has been resolved ---- \greg{(a) and (b) don't have the same bandwidth, so (c) is confusing because the time indexes are not aligned for the three signals. Could we overlap the filtered/decimated LTE spectrum on top of (b)?}}
\label{fig:uplink_rqf}
\vspace{-15pt}
\end{figure*}

\end{comment}


